On the Extension of a Physical Body in Classical Motion. An Analogy for a Pseudo-Velocity Concept and Wiener's Process in (Ideal) Polymer Solutions

A pseudo-velocity concept, based on the extension of a linear body, is defined by a special relativity experiment. It suggests an analogy with the covariance properties of Wiener's process, ultimately implying that the scaling behavior of (Gaussian) polymer solutions can be derived from a Brownian Relativity theory, as it was formerly put forward. An ad-hoc statistical interpretation of the resulting spacetime transforms may be given by the central limit theorem.

==> RevTeX 4.2 Template and Sample/bib2.tex <==
@PREAMBLE{
 "\providecommand{\noopsort}[1]{}" 
 # "\providecommand{\singleletter}[1]{#1}%" 
}

@ARTICLE{ver16,
author="Verhille, Gautier
and Bartoli, Adrien",
title="3D conformation of a flexible fiber in a turbulent flow",
journal="Exp. Fluids",
year="2016",
month="Jun",
day="23",
volume="57",
number="7",
pages="117",
issn="1432-1114",
doi="10.1007/s00348-016-2201-1",
url="https://doi.org/10.1007/s00348-016-2201-1"
}

@BOOK{sam1,
author = "S. A. Mezzasalma",
publisher = "Academic Press-Elsevier, London",
pages = "ix + 236",
year = "2008",
booktitle = "Macromolecules in Solution and Brownian Relativity",
issn = "1573-4285",
doi = "https://doi.org/10.1016/S1573-4285(07)00009-9",
}

@ARTICLE{sam2,
author = {Mezzasalma, Stefano A.},
journal = {Langmuir},
title = {Long-range correlations, geometrical structure, and transport properties of macromolecular solutions. The equivalence of configurational statistics and geometrodynamics of large molecules},
volume = {23},
number = {25},
pages = {12737-12751},
year = {2007},
doi = {10.1021/la701891m},
}

@ARTICLE{sam3,
journal = "J. Colloid Interface Sci.",
volume = "307",
title = "The special theory of Brownian relativity: Equivalence principle for dynamic and static random paths and uncertainty relation for diffusion",
number = "2",
pages = "386-397",
year = "2007",
doi = "https://doi.org/10.1016/j.jcis.2006.11.042",
author = "S. Mezzasalma",
}
@ARTICLE{sam4,
author = {Mezzasalma, Stefano A.},
journal = {J. Phys. Chem. B},
title = {Configurational Statistics of Macromolecules in Solution from Correlations of Liquid Molecules},
volume = {110},
number = {46},
pages = {23507-23514},
year = {2006},
doi = {10.1021/jp063539d},
}

@ARTICLE{sam5,
journal = "Chem. Phys.",
volume = "334",
title = "Anomalous scaling in passive scalar advection from anomalous exponents in polymer partition function",
number = "1",
pages = "232 - 241",
year = "2007",
issn = "0301-0104",
doi = "https://doi.org/10.1016/j.chemphys.2007.03.008",
author = "Stefano A. Mezzasalma",
}

@BOOK{pierre79,
  added-at = {2010-11-05T11:32:43.000+0100},
  address = {Ithaca},
  author = {de Gennes, P.G.},
  isbn = {0-8014-1203-X},
  pages = {324},
  publisher = {Cornell University Press},
  title = {Scaling concepts in polymer physics},
  year = 1979
}

@ARTICLE{nie82,
  author = {Nienhuis, Bernard},
  journal = {Phys. Rev. Lett.},
  volume = {49},
  title = {Exact Critical Point and Critical Exponents of O(n) Models in Two Dimensions},
  issue = {15},
  pages = {1062--1065},
  numpages = {0},
  year = {1982},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.49.1062},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.49.1062}
}

@BOOK{rub03,
  title={Polymer Physics},
  author={Rubinstein, M. and Colby, R.H.},
  isbn={9781613449431},
  year={2003},
  pages = {440},
  publisher={Oxford University Press}
}

@ARTICLE{bro14,
  author = {Brouzet, C. and Verhille, G. and Le Gal, P.},
  journal = {Phys. Rev. Lett.},
  volume = {112},
  title = {Flexible Fiber in a Turbulent Flow: A Macroscopic Polymer},
  issue = {7},
  pages = {074501},
  numpages = {5},
  year = {2014},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.112.074501},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.112.074501},
}

@ARTICLE{theo17,
issn = {0378-4371},
journal = {Physica A},
title = {Material line fluctuations slaved to bulk correlations in two-dimensional turbulence},
pages = {180--183},
volume = {467},
publisher = {Elsevier Science},
year = {2017},
author = {Odijk, Theo},
}

@article{sam7,
title = "Universality in polymer solutions from intrinsic viscosity as a Lorentz factor",
journal = "Chem. Phys. Lett.",
volume = "403",
number = "4",
pages = "334 - 337",
year = "2005",
issn = "0009-2614",
doi = "https://doi.org/10.1016/j.cplett.2005.01.027",
author = "Stefano A. Mezzasalma",
}

@ARTICLE{nov15,
author = {Le Nov\'ere, N.},
year = {2015},
month = {02},
pages = {146 -- 158},
title = {Quantitative and logic modelling of molecular and gene networks},
volume = {16},
journal = {Nat. Rev. Genet.},
doi = {10.1038/nrg3885}
}

@INCOLLECTION{cow12,
title = "Chapter 8 - Spatial Modeling of Cell Signaling Networks",
editor = "Anand R. Asthagiri and Adam P. Arkin",
series = "Methods in Cell Biology",
publisher = "Academic Press",
volume = "110",
pages = "195 - 221",
year = "2012",
booktitle = "Computational Methods in Cell Biology",
doi = "https://doi.org/10.1016/B978-0-12-388403-9.00008-4",
url = "http://www.sciencedirect.com/science/article/pii/B9780123884039000084",
author = "Ann E. Cowan and Ion I. Moraru and James C. Schaff and Boris M. Slepchenko and Leslie M. Loew",
}

@ARTICLE{isaac09,
author = {Isaacson, Samuel A.},
title = {The Reaction-Diffusion Master Equation as an Asymptotic Approximation of Diffusion to a Small Target},
journal = {SIAM J. Appl. Math.},
volume = {70},
number = {1},
pages = {77-111},
year = {2009},
doi = {10.1137/070705039},
}

@ARTICLE{gil07,
author = {Gillespie, Daniel T.},
title = {Stochastic Simulation of Chemical Kinetics},
journal = {Annual Review of Physical Chemistry},
volume = {58},
number = {1},
pages = {35-55},
year = {2007},
doi = {10.1146/annurev.physchem.58.032806.104637},
}

@book{mis17,
  title={Gravitation},
  author={Misner, C.W. and Thorne, K.S. and Wheeler, J.A. and Kaiser, D.I.},
  year={2017},
  publisher={Princeton University Press}
}

@book{van07,
  author = {Kampen, NG Van},
  publisher = {North Holland},
  timestamp = {2010-06-08T20:50:38.000+0200},
  title = {Stochastic processes in physics and chemistry},
  year = 2007
}

@article{sam6,
author = {Mezzasalma, S.A.},
year = {2005},
month = {08},
pages = {408-418},
title = {Chain propagator, mass, and universality in polymer solutions from Brownian relativity},
volume = {318},
journal = {Annals of Physics},
doi = {10.1016/j.aop.2005.01.007}
}

@book{brz00,
  author = {Brze{\'z}niak, Zdzis{\l}aw and Zastawniak, Tomasz},
  publisher = {Springer},
  timestamp = {2009-10-28T04:43:05.000+0100},
  title = {Basic Stochastic Processes},
  year = 2000
}

@book{ein56,
  title={Investigations on the Theory of the Brownian Movement},
  author={Einstein, A.},
  isbn={9780486603049},
  series={Dover Books on Physics Series},
  url={https://books.google.hr/books?id=AOIVupH\_hboC},
  year={1956},
  publisher={Dover Publications}
}


@ARTICLE{feyn54,
   author       = "R. P. Feynman",
   year         = "1954",
   journal      = "Phys.\ Rev.",
   volume       = "94",
   pages        = "262",
}

@ARTICLE{epr,
   author       = "A. Einstein and {\relax Yu} Podolsky and N. Rosen", 
   collaboration = "EPR",
   year         = "1935", 
   journal      = "Phys.\ Rev.", 
   volume       = "47", 
   pages        = "777",
}

@MISC{witten2001,
   author       = "Edward Witten",
   eprint       = "hep-th/0106109",
   year         = "2001",
}

@INBOOK{Beutler1994,
   author       = "E. Beutler", 
   editor       = "E. Beutler and M. A. Lichtman and B. W. Coller and T. S. Kipps", 
   booktitle    = "Williams Hematology", 
   chapter      = "7", 
   pages        = "654--662",
   publisher    = "McGraw-Hill", 
   year         = "1994", 

   edition      = "5", 
   address      = "New York", 
   volume       = "2", 
}

@INCOLLECTION{Beutler1994a,
   author       = "E. Beutler", 
   editor       = "E. Beutler and M. A. Lichtman and B. W. Coller and T. S. Kipps", 
   booktitle    = "Williams Hematology", 
   chapter      = "7", 
   pages        = "654--662",
   publisher    = "McGraw-Hill", 
   year         = "1994", 

   edition      = "5", 
   address      = "New York", 
   volume       = "2", 
}

@INBOOK{inbook-full,
   author    = "Donald E. Knuth",
   booktitle = "Fundamental Algorithms",
   volume    = 1,
   series    = "The Art of Computer Programming",
   publisher = "Addison-Wesley",
   address   = "Reading, Massachusetts",
   edition   = "Second",
   month     = "10~" # jan,
   year      = "\noopsort{1973b}1973",
   type      = "Section",
   chapter   = "1.2",
   pages     = "10--119",
   note      = "A full INBOOK entry",
}

@UNPUBLISHED{Smith2010,
   author       = "W. J. Smith and T. J. Johnson and B. G. Miller", 
   title        = "Surface chemistry and preferential crystal orientation on a silicon surface", 
   note         = "{J. Appl. Phys.} (unpublished)", 
   
   month        = "", 
   year         = "2010",
}

@UNPUBLISHED{unpublished-full,
   author = "Ulrich {\"{U}}nderwood and Ned {\~N}et and Paul {\={P}}ot",
   title = "Lower Bounds for Wishful Research Results",
   month = nov # ", " # dec,
   year = 1988,
   note = "Talk at Fanstord University (A full UNPUBLISHED entry)",
}

@MISC{JohnsonMillerSmith2007, 

   author       = "M. P. Johnson and K. L. Miller and K. Smith", 
   title        = "", 
   howpublished = "personal communication", 
   month        = "1~" # may, 
   year         = "2007", 
   note         = "",
}

@PROCEEDINGS{Smith2007, 
   title        = "AIP Conf. Proc.", 
   year         = "2007", 
   
   editor       = "J. Smith", 
   volume       = "841", 
   number       = "21", 
   series       = "", 
   address      = "", 
   month        = "", 
   organization = "", 
   publisher    = "", 
   note         = "", 
}

@PROCEEDINGS{proceedings-full,
   editor = "Wizard V. Oz and Mihalis Yannakakis",
   title = "Proc. Fifteenth Annual",
   number = 17,
   series = "All ACM Conferences",
   month = mar,
   year = 1983,
   address = "Boston",
   organization = "ACM",
   publisher = "Academic Press",
   note = "A full PROCEEDINGS entry",
}

@PROCEEDINGS{Quinn2001, 
   title        = "{Proceedings of the 2003 Particle  Accelerator Conference, Portland, OR, 12-16 May 2005}", 
   year         = "2001", 
   
   editor       = "B. Quinn", 
   address      = "New York", 
   publisher    = "Wiley", 
   note         = "Albeit the conference was held in 2005, it was the 2003 conference, and  the proceedings were published in 2001; go figure", 
}

@TECHREPORT{techreport-full,
   author = "Tom T{\'{e}}rrific",
   title = "An {$O(n \log n / \! \log\log n)$} Sorting Algorithm",
   institution = "Fanstord University",
   type = "Wishful Research Result",
   number = "7",
   address = "Computer Science Department, Fanstord, California",
   month = oct,
   year = 1988,
   note = "A full TECHREPORT entry",
}

@TECHREPORT{Nelson1999, 
   author       = "J. Nelson", 
   type         = "{TWI Report}", 
   number       = "666/1999",
   institution  = "", 
   year         = jan # "~1999", 
   
   note         = "Required institution missing", 
}

@MISC{Zalkins2008, 

   author       = "Y. M. Zalkins", 
   title        = "", 
   howpublished = "e-print arXiv:cond-mat/040426", 
   month        = "", 
   year         = "2008", 
   note         = "",
}

@MISC{Nelson2005, 

   author       = "J. Nelson", 
   howpublished = "{U.S. Patent No.} 5,693,000", 
   year         = "12~" # dec # "~2005", 
}

@MASTERSTHESIS{Nelson1999a,
   author       = "J. K. Nelson", 
   title        = "", 
   school       = "New York University", 
   year         = "1999", 
   
   type         = "M.{S}. thesis", 
   address      = "", 
   month        = "", 
   note         = "", 
}

@MASTERSTHESIS{mastersthesis-full,
   author = "{\'{E}}douard Masterly",
   title = "Mastering Thesis Writing",
   school = "Stanford University",
   type = "Master's project",
   address = "English Department",
   month = jun # "-" # aug,
   year = 1988,
   note = "A full MASTERSTHESIS entry",
}

@PHDTHESIS{Smith2003,
   author       = "S. M. Smith", 
   title        = "", 
   school       = "Massachusetts Institute of  Technology", 
   year         = "2003", 
   
   type         = "{Ph.D.} thesis", 
   address      = "", 
   month        = "", 
   note         = "", 
}

@PHDTHESIS{phdthesis-full,
   author = "F. Phidias Phony-Baloney",
   title = "Fighting Fire with Fire: Festooning {F}rench Phrases",
   school = "Fanstord University",
   type = "{PhD} Dissertation",
   address = "Department of French",
   month = jun # "-" # aug,
   year = 1988,
   note = "A full PHDTHESIS entry",
}

@BOOK{book-full,
   author = "Donald E. Knuth",
   title = "Seminumerical Algorithms",
   volume = 2,
   series = "The Art of Computer Programming",
   publisher = "Addison-Wesley",
   address = "Reading, Massachusetts",
   edition = "Second",
   month = "10~" # jan,
   year = "\noopsort{1973c}1981",
   note = "A full BOOK entry",
}

@BOOKLET{booklet-full,
   author = "Jill C. Knvth",
   title = "The Programming of Computer Art",
   howpublished = "Vernier Art Center",
   address = "Stanford, California",
   month = feb,
   year = 1988,
   note = "A full BOOKLET entry",
}

@INBOOK{ballagh2000,
   author    = "R. Ballagh and C.M. Savage",
   editor    = "C.M. Savage and M. Das",
   title     = "Bose-Einstein condensation: from atomic physics to quantum fluids, Proceedings of the 13th Physics Summer School",
   year      = "2000",
   publisher = "World Scientific",
   address   = "Singapore",
   eprint    = "cond-mat/0008070",
}

@INCOLLECTION{ballagh2000a,
   author    = "R. Ballagh and C.M. Savage",
   title     = "Bose-Einstein condensation: from atomic physics to quantum fluids",
   editor    = "C.M. Savage and M. Das",
   booktitle = "Proceedings of the 13th Physics Summer School",
   year      = "2000",
   publisher = "World Scientific",
   address   = "Singapore",
   eprint    = "cond-mat/0008070",
}

@inBook{Magnetism,
   author    = "W. Opechowski and R. Guccione",
   title     = "Introduction to the Theory of Normal Metals",
   volume    = "IIa",
   pages     = "105",
   editor    = "G. T. Rado and H. Suhl",
   booktitle = "Magnetism",
   publisher = "Academic Press",
   address   = "New York",
   year      = "1965",
}

@INCOLLECTION{Magnetisma,
   author    = "W. Opechowski and R. Guccione",
   title     = "Introduction to the Theory of Normal Metals",
   editor    = "G. T. Rado and H. Suhl",
   booktitle = "Magnetism",
   volume    = "IIa",
   pages     = "105",
   publisher = "Academic Press",
   address   = "New York",
   year      = "1965",
}

@INPROCEEDINGS{Magnetismb,
   author    = "W. Opechowski and R. Guccione",
   title     = "Introduction to the Theory of Normal Metals",
   editor    = "G. T. Rado and H. Suhl",
   booktitle = "Magnetism",
   volume    = "IIa",
   pages     = "105",
   publisher = "Academic Press",
   address   = "New York",
   year      = "1965",
}

@article{ZS71,
   author    = "V. E. Zakharov and A. B. Shabat",
   title     = "Exact theory of two-dimensional self-focusing and one-dimensional self-modulation of waves in nonlinear media",
   journal   = "Zh. Eksp. Teor. Fiz.",
   volume    = "61",
   year      = "1971",
   pages     = "118--134",
   translation = "Sov. Phys. JETP \textbf{34}, 62 (1972)"
}

@INCOLLECTION{incollection-full,
   author = "Daniel D. Lincoll",
   title = "Semigroups of Recurrences",
   editor = "David J. Lipcoll and D. H. Lawrie and A. H. Sameh",
   booktitle = "High Speed Computer and Algorithm Organization",
   number = 23,
   series = "Fast Computers",
   chapter = 3,
   type = "Part",
   pages = "179--183",
   publisher = "Academic Press",
   address = "New York",
   edition = "Third",
   month = sep,
   year = 1977,
   note = "A full INCOLLECTION entry",
}

@INPROCEEDINGS{inproceedings-full,
   author = "Alfred V. Oaho and Jeffrey D. Ullman and Mihalis Yannakakis",
   title = "On Notions of Information Transfer in {VLSI} Circuits",
   editor = "Wizard V. Oz and Mihalis Yannakakis",
   booktitle = "Proc. Fifteenth Annual ACM",
   bookaddress = "Boston, 1982", 
   number = 17,
   series = "All ACM Conferences",
   pages = "133--139",
   month = mar,
   year = 1983,
   address = "New York",
   organization = "ACM",
   publisher = "Academic Press",
   note = "A full INPROCEDINGS entry",
}

@MANUAL{manual-full,
   author = "Larry Manmaker",
   title = "The Definitive Computer Manual",
   organization = "Chips-R-Us",
   address = "Silicon Valley",
   edition = "Silver",
   month = apr # "-" # may,
   year = 1986,
   note = "A full MANUAL entry",
}

@book{nel67,
  title={Dynamical Theories of Brownian Motion},
  author={Nelson, E.},
  isbn={9780691079509},
  lccn={72038239},
  series={Mathematical Notes - Princeton University Press},
  url={https://books.google.it/books?id=xuQ9DwAAQBAJ},
  year={1967},
  publisher={Princeton University Press}
}


==> bib2.tex <==
@PREAMBLE{
 "\providecommand{\noopsort}[1]{}" 
 # "\providecommand{\singleletter}[1]{#1}%" 
}

@ARTICLE{ver16,
author="Verhille, Gautier
and Bartoli, Adrien",
title="3D conformation of a flexible fiber in a turbulent flow",
journal="Exp. Fluids",
year="2016",
month="Jun",
day="23",
volume="57",
number="7",
pages="117",
issn="1432-1114",
doi="10.1007/s00348-016-2201-1",
url="https://doi.org/10.1007/s00348-016-2201-1"
}

@BOOK{sam1,
author = "S. A. Mezzasalma",
publisher = "Academic Press-Elsevier, London",
pages = "ix + 236",
year = "2008",
booktitle = "Macromolecules in Solution and Brownian Relativity",
issn = "1573-4285",
doi = "https://doi.org/10.1016/S1573-4285(07)00009-9",
}

@ARTICLE{sam2,
author = {Mezzasalma, Stefano A.},
journal = {Langmuir},
title = {Long-range correlations, geometrical structure, and transport properties of macromolecular solutions. The equivalence of configurational statistics and geometrodynamics of large molecules},
volume = {23},
number = {25},
pages = {12737-12751},
year = {2007},
doi = {10.1021/la701891m},
}

@ARTICLE{sam3,
journal = "J. Colloid Interface Sci.",
volume = "307",
title = "The special theory of Brownian relativity: Equivalence principle for dynamic and static random paths and uncertainty relation for diffusion",
number = "2",
pages = "386-397",
year = "2007",
doi = "https://doi.org/10.1016/j.jcis.2006.11.042",
author = "S. Mezzasalma",
}
@ARTICLE{sam4,
author = {Mezzasalma, Stefano A.},
journal = {J. Phys. Chem. B},
title = {Configurational Statistics of Macromolecules in Solution from Correlations of Liquid Molecules},
volume = {110},
number = {46},
pages = {23507-23514},
year = {2006},
doi = {10.1021/jp063539d},
}

@ARTICLE{sam5,
journal = "Chem. Phys.",
volume = "334",
title = "Anomalous scaling in passive scalar advection from anomalous exponents in polymer partition function",
number = "1",
pages = "232 - 241",
year = "2007",
issn = "0301-0104",
doi = "https://doi.org/10.1016/j.chemphys.2007.03.008",
author = "Stefano A. Mezzasalma",
}

@BOOK{pierre79,
  added-at = {2010-11-05T11:32:43.000+0100},
  address = {Ithaca},
  author = {de Gennes, P.G.},
  isbn = {0-8014-1203-X},
  pages = {324},
  publisher = {Cornell University Press},
  title = {Scaling concepts in polymer physics},
  year = 1979
}

@ARTICLE{nie82,
  author = {Nienhuis, Bernard},
  journal = {Phys. Rev. Lett.},
  volume = {49},
  title = {Exact Critical Point and Critical Exponents of O(n) Models in Two Dimensions},
  issue = {15},
  pages = {1062--1065},
  numpages = {0},
  year = {1982},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.49.1062},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.49.1062}
}

@BOOK{rub03,
  title={Polymer Physics},
  author={Rubinstein, M. and Colby, R.H.},
  isbn={9781613449431},
  year={2003},
  pages = {440},
  publisher={Oxford University Press}
}

@ARTICLE{bro14,
  author = {Brouzet, C. and Verhille, G. and Le Gal, P.},
  journal = {Phys. Rev. Lett.},
  volume = {112},
  title = {Flexible Fiber in a Turbulent Flow: A Macroscopic Polymer},
  issue = {7},
  pages = {074501},
  numpages = {5},
  year = {2014},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.112.074501},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.112.074501},
}

@ARTICLE{theo17,
issn = {0378-4371},
journal = {Physica A},
title = {Material line fluctuations slaved to bulk correlations in two-dimensional turbulence},
pages = {180--183},
volume = {467},
publisher = {Elsevier Science},
year = {2017},
author = {Odijk, Theo},
}

@article{sam7,
title = "Universality in polymer solutions from intrinsic viscosity as a Lorentz factor",
journal = "Chem. Phys. Lett.",
volume = "403",
number = "4",
pages = "334 - 337",
year = "2005",
issn = "0009-2614",
doi = "https://doi.org/10.1016/j.cplett.2005.01.027",
author = "Stefano A. Mezzasalma",
}

@ARTICLE{nov15,
author = {Le Nov\'ere, N.},
year = {2015},
month = {02},
pages = {146 -- 158},
title = {Quantitative and logic modelling of molecular and gene networks},
volume = {16},
journal = {Nat. Rev. Genet.},
doi = {10.1038/nrg3885}
}

@INCOLLECTION{cow12,
title = "Chapter 8 - Spatial Modeling of Cell Signaling Networks",
editor = "Anand R. Asthagiri and Adam P. Arkin",
series = "Methods in Cell Biology",
publisher = "Academic Press",
volume = "110",
pages = "195 - 221",
year = "2012",
booktitle = "Computational Methods in Cell Biology",
doi = "https://doi.org/10.1016/B978-0-12-388403-9.00008-4",
url = "http://www.sciencedirect.com/science/article/pii/B9780123884039000084",
author = "Ann E. Cowan and Ion I. Moraru and James C. Schaff and Boris M. Slepchenko and Leslie M. Loew",
}

@ARTICLE{isaac09,
author = {Isaacson, Samuel A.},
title = {The Reaction-Diffusion Master Equation as an Asymptotic Approximation of Diffusion to a Small Target},
journal = {SIAM J. Appl. Math.},
volume = {70},
number = {1},
pages = {77-111},
year = {2009},
doi = {10.1137/070705039},
}

@ARTICLE{gil07,
author = {Gillespie, Daniel T.},
title = {Stochastic Simulation of Chemical Kinetics},
journal = {Annual Review of Physical Chemistry},
volume = {58},
number = {1},
pages = {35-55},
year = {2007},
doi = {10.1146/annurev.physchem.58.032806.104637},
}

@book{mis17,
  title={Gravitation},
  author={Misner, C.W. and Thorne, K.S. and Wheeler, J.A. and Kaiser, D.I.},
  year={2017},
  publisher={Princeton University Press}
}

@book{van07,
  author = {Kampen, NG Van},
  publisher = {North Holland},
  timestamp = {2010-06-08T20:50:38.000+0200},
  title = {Stochastic processes in physics and chemistry},
  year = 2007
}

@article{sam6,
author = {Mezzasalma, S.A.},
year = {2005},
month = {08},
pages = {408-418},
title = {Chain propagator, mass, and universality in polymer solutions from Brownian relativity},
volume = {318},
journal = {Annals of Physics},
doi = {10.1016/j.aop.2005.01.007}
}

@book{brz00,
  author = {Brze{\'z}niak, Zdzis{\l}aw and Zastawniak, Tomasz},
  publisher = {Springer},
  timestamp = {2009-10-28T04:43:05.000+0100},
  title = {Basic Stochastic Processes},
  year = 2000
}

@book{ein56,
  title={Investigations on the Theory of the Brownian Movement},
  author={Einstein, A.},
  isbn={9780486603049},
  series={Dover Books on Physics Series},
  url={https://books.google.hr/books?id=AOIVupH\_hboC},
  year={1956},
  publisher={Dover Publications}
}


@ARTICLE{feyn54,
   author       = "R. P. Feynman",
   year         = "1954",
   journal      = "Phys.\ Rev.",
   volume       = "94",
   pages        = "262",
}

@ARTICLE{epr,
   author       = "A. Einstein and {\relax Yu} Podolsky and N. Rosen", 
   collaboration = "EPR",
   year         = "1935", 
   journal      = "Phys.\ Rev.", 
   volume       = "47", 
   pages        = "777",
}

@MISC{witten2001,
   author       = "Edward Witten",
   eprint       = "hep-th/0106109",
   year         = "2001",
}

@INBOOK{Beutler1994,
   author       = "E. Beutler", 
   editor       = "E. Beutler and M. A. Lichtman and B. W. Coller and T. S. Kipps", 
   booktitle    = "Williams Hematology", 
   chapter      = "7", 
   pages        = "654--662",
   publisher    = "McGraw-Hill", 
   year         = "1994", 

   edition      = "5", 
   address      = "New York", 
   volume       = "2", 
}

@INCOLLECTION{Beutler1994a,
   author       = "E. Beutler", 
   editor       = "E. Beutler and M. A. Lichtman and B. W. Coller and T. S. Kipps", 
   booktitle    = "Williams Hematology", 
   chapter      = "7", 
   pages        = "654--662",
   publisher    = "McGraw-Hill", 
   year         = "1994", 

   edition      = "5", 
   address      = "New York", 
   volume       = "2", 
}

@INBOOK{inbook-full,
   author    = "Donald E. Knuth",
   booktitle = "Fundamental Algorithms",
   volume    = 1,
   series    = "The Art of Computer Programming",
   publisher = "Addison-Wesley",
   address   = "Reading, Massachusetts",
   edition   = "Second",
   month     = "10~" # jan,
   year      = "\noopsort{1973b}1973",
   type      = "Section",
   chapter   = "1.2",
   pages     = "10--119",
   note      = "A full INBOOK entry",
}

@UNPUBLISHED{Smith2010,
   author       = "W. J. Smith and T. J. Johnson and B. G. Miller", 
   title        = "Surface chemistry and preferential crystal orientation on a silicon surface", 
   note         = "{J. Appl. Phys.} (unpublished)", 
   
   month        = "", 
   year         = "2010",
}

@UNPUBLISHED{unpublished-full,
   author = "Ulrich {\"{U}}nderwood and Ned {\~N}et and Paul {\={P}}ot",
   title = "Lower Bounds for Wishful Research Results",
   month = nov # ", " # dec,
   year = 1988,
   note = "Talk at Fanstord University (A full UNPUBLISHED entry)",
}

@MISC{JohnsonMillerSmith2007, 

   author       = "M. P. Johnson and K. L. Miller and K. Smith", 
   title        = "", 
   howpublished = "personal communication", 
   month        = "1~" # may, 
   year         = "2007", 
   note         = "",
}

@PROCEEDINGS{Smith2007, 
   title        = "AIP Conf. Proc.", 
   year         = "2007", 
   
   editor       = "J. Smith", 
   volume       = "841", 
   number       = "21", 
   series       = "", 
   address      = "", 
   month        = "", 
   organization = "", 
   publisher    = "", 
   note         = "", 
}

@PROCEEDINGS{proceedings-full,
   editor = "Wizard V. Oz and Mihalis Yannakakis",
   title = "Proc. Fifteenth Annual",
   number = 17,
   series = "All ACM Conferences",
   month = mar,
   year = 1983,
   address = "Boston",
   organization = "ACM",
   publisher = "Academic Press",
   note = "A full PROCEEDINGS entry",
}

@PROCEEDINGS{Quinn2001, 
   title        = "{Proceedings of the 2003 Particle  Accelerator Conference, Portland, OR, 12-16 May 2005}", 
   year         = "2001", 
   
   editor       = "B. Quinn", 
   address      = "New York", 
   publisher    = "Wiley", 
   note         = "Albeit the conference was held in 2005, it was the 2003 conference, and  the proceedings were published in 2001; go figure", 
}

@TECHREPORT{techreport-full,
   author = "Tom T{\'{e}}rrific",
   title = "An {$O(n \log n / \! \log\log n)$} Sorting Algorithm",
   institution = "Fanstord University",
   type = "Wishful Research Result",
   number = "7",
   address = "Computer Science Department, Fanstord, California",
   month = oct,
   year = 1988,
   note = "A full TECHREPORT entry",
}

@TECHREPORT{Nelson1999, 
   author       = "J. Nelson", 
   type         = "{TWI Report}", 
   number       = "666/1999",
   institution  = "", 
   year         = jan # "~1999", 
   
   note         = "Required institution missing", 
}

@MISC{Zalkins2008, 

   author       = "Y. M. Zalkins", 
   title        = "", 
   howpublished = "e-print arXiv:cond-mat/040426", 
   month        = "", 
   year         = "2008", 
   note         = "",
}

@MISC{Nelson2005, 

   author       = "J. Nelson", 
   howpublished = "{U.S. Patent No.} 5,693,000", 
   year         = "12~" # dec # "~2005", 
}

@MASTERSTHESIS{Nelson1999a,
   author       = "J. K. Nelson", 
   title        = "", 
   school       = "New York University", 
   year         = "1999", 
   
   type         = "M.{S}. thesis", 
   address      = "", 
   month        = "", 
   note         = "", 
}

@MASTERSTHESIS{mastersthesis-full,
   author = "{\'{E}}douard Masterly",
   title = "Mastering Thesis Writing",
   school = "Stanford University",
   type = "Master's project",
   address = "English Department",
   month = jun # "-" # aug,
   year = 1988,
   note = "A full MASTERSTHESIS entry",
}

@PHDTHESIS{Smith2003,
   author       = "S. M. Smith", 
   title        = "", 
   school       = "Massachusetts Institute of  Technology", 
   year         = "2003", 
   
   type         = "{Ph.D.} thesis", 
   address      = "", 
   month        = "", 
   note         = "", 
}

@PHDTHESIS{phdthesis-full,
   author = "F. Phidias Phony-Baloney",
   title = "Fighting Fire with Fire: Festooning {F}rench Phrases",
   school = "Fanstord University",
   type = "{PhD} Dissertation",
   address = "Department of French",
   month = jun # "-" # aug,
   year = 1988,
   note = "A full PHDTHESIS entry",
}

@BOOK{book-full,
   author = "Donald E. Knuth",
   title = "Seminumerical Algorithms",
   volume = 2,
   series = "The Art of Computer Programming",
   publisher = "Addison-Wesley",
   address = "Reading, Massachusetts",
   edition = "Second",
   month = "10~" # jan,
   year = "\noopsort{1973c}1981",
   note = "A full BOOK entry",
}

@BOOKLET{booklet-full,
   author = "Jill C. Knvth",
   title = "The Programming of Computer Art",
   howpublished = "Vernier Art Center",
   address = "Stanford, California",
   month = feb,
   year = 1988,
   note = "A full BOOKLET entry",
}

@INBOOK{ballagh2000,
   author    = "R. Ballagh and C.M. Savage",
   editor    = "C.M. Savage and M. Das",
   title     = "Bose-Einstein condensation: from atomic physics to quantum fluids, Proceedings of the 13th Physics Summer School",
   year      = "2000",
   publisher = "World Scientific",
   address   = "Singapore",
   eprint    = "cond-mat/0008070",
}

@INCOLLECTION{ballagh2000a,
   author    = "R. Ballagh and C.M. Savage",
   title     = "Bose-Einstein condensation: from atomic physics to quantum fluids",
   editor    = "C.M. Savage and M. Das",
   booktitle = "Proceedings of the 13th Physics Summer School",
   year      = "2000",
   publisher = "World Scientific",
   address   = "Singapore",
   eprint    = "cond-mat/0008070",
}

@inBook{Magnetism,
   author    = "W. Opechowski and R. Guccione",
   title     = "Introduction to the Theory of Normal Metals",
   volume    = "IIa",
   pages     = "105",
   editor    = "G. T. Rado and H. Suhl",
   booktitle = "Magnetism",
   publisher = "Academic Press",
   address   = "New York",
   year      = "1965",
}

@INCOLLECTION{Magnetisma,
   author    = "W. Opechowski and R. Guccione",
   title     = "Introduction to the Theory of Normal Metals",
   editor    = "G. T. Rado and H. Suhl",
   booktitle = "Magnetism",
   volume    = "IIa",
   pages     = "105",
   publisher = "Academic Press",
   address   = "New York",
   year      = "1965",
}

@INPROCEEDINGS{Magnetismb,
   author    = "W. Opechowski and R. Guccione",
   title     = "Introduction to the Theory of Normal Metals",
   editor    = "G. T. Rado and H. Suhl",
   booktitle = "Magnetism",
   volume    = "IIa",
   pages     = "105",
   publisher = "Academic Press",
   address   = "New York",
   year      = "1965",
}

@article{ZS71,
   author    = "V. E. Zakharov and A. B. Shabat",
   title     = "Exact theory of two-dimensional self-focusing and one-dimensional self-modulation of waves in nonlinear media",
   journal   = "Zh. Eksp. Teor. Fiz.",
   volume    = "61",
   year      = "1971",
   pages     = "118--134",
   translation = "Sov. Phys. JETP \textbf{34}, 62 (1972)"
}

@INCOLLECTION{incollection-full,
   author = "Daniel D. Lincoll",
   title = "Semigroups of Recurrences",
   editor = "David J. Lipcoll and D. H. Lawrie and A. H. Sameh",
   booktitle = "High Speed Computer and Algorithm Organization",
   number = 23,
   series = "Fast Computers",
   chapter = 3,
   type = "Part",
   pages = "179--183",
   publisher = "Academic Press",
   address = "New York",
   edition = "Third",
   month = sep,
   year = 1977,
   note = "A full INCOLLECTION entry",
}

@INPROCEEDINGS{inproceedings-full,
   author = "Alfred V. Oaho and Jeffrey D. Ullman and Mihalis Yannakakis",
   title = "On Notions of Information Transfer in {VLSI} Circuits",
   editor = "Wizard V. Oz and Mihalis Yannakakis",
   booktitle = "Proc. Fifteenth Annual ACM",
   bookaddress = "Boston, 1982", 
   number = 17,
   series = "All ACM Conferences",
   pages = "133--139",
   month = mar,
   year = 1983,
   address = "New York",
   organization = "ACM",
   publisher = "Academic Press",
   note = "A full INPROCEDINGS entry",
}

@MANUAL{manual-full,
   author = "Larry Manmaker",
   title = "The Definitive Computer Manual",
   organization = "Chips-R-Us",
   address = "Silicon Valley",
   edition = "Silver",
   month = apr # "-" # may,
   year = 1986,
   note = "A full MANUAL entry",
}

@book{nel67,
  title={Dynamical Theories of Brownian Motion},
  author={Nelson, E.},
  isbn={9780691079509},
  lccn={72038239},
  series={Mathematical Notes - Princeton University Press},
  url={https://books.google.it/books?id=xuQ9DwAAQBAJ},
  year={1967},
  publisher={Princeton University Press}
}

